The Lyman Alpha Spectral Database (LASD)

Lyman $\alpha$ (Ly$\alpha$) emission from star-forming galaxies is an important tool to study a large range of astrophysical questions: it has the potential to carry information about the source galaxy, its nearby circumgalactic medium, and also the surrounding intergalactic medium. Much observational and theoretical work has therefore focused on understanding the details of this emission line. These efforts have been hampered, however, by an absence of spectroscopic reference samples that can be used both as comparisons for observational studies and as critical tests for theoretical work. For this reason we have compiled a large sample of Ly$\alpha$ spectra, at both low and high redshift, and created a publicly available online database, at http://lasd.lyman-alpha.com. The Lyman alpha Spectral Database (LASD) hosts these spectra, as well as large set of spectral and kinematic quantities that have been homogeneously measured for the entire sample. These can easily be viewed online and downloaded in tabular form. The LASD has the capacity for users to easily upload their own Ly$\alpha$ spectra, and all the same spectral measurements will be made, reported, and ingested into the database. We actively invite the community to do so, and the LASD is intended to be a long-term community resource. In this paper we present the design of the database as well as descriptions of the underlying algorithms and the initial Ly$\alpha$ emitter samples that are in the database.

==> LASD Paper ArXiv Version/includes/description.tex <==
%%% This is an automatically generated file. Change manually at own risk!
\begin{tabular}{lp{9cm}l}
\toprule
                         Name &                                                                          Description &         Units \\
\midrule
             \texttt{Dx\_max} &                                Peak separation between maximum luminosity densities &          km/s \\
            \texttt{Dx\_mean} &                                 Peak separation between first moments of both sides &          km/s \\
                  \texttt{EW} &                                                            Restframe quivalent width of line &             \AA \\
           \texttt{FWHM\_max} &                                          Full-width at half maximum of highest peak &          km/s \\
           \texttt{FWHM\_neg} &                                             Full-width at half maximum of blue side &          km/s \\
           \texttt{FWHM\_pos} &                                              Full-width at half maximum of red side &          km/s \\
             \texttt{F\_cont} &                                                                  Level of continuum &  erg/s/(km/s) \\
               \texttt{F\_lc} &                                                   Luminosity density at line center &  erg/s/(km/s) \\
              \texttt{F\_max} &                                                  Luminosity density of highest peak &  erg/s/(km/s) \\
         \texttt{F\_neg\_max} &                                     Luminosity density of highest peak on blue side &  erg/s/(km/s) \\
         \texttt{F\_pos\_max} &                                      Luminosity density of highest peak on red side &  erg/s/(km/s) \\
           \texttt{F\_valley} &                                         Luminosity density of minimum between peaks &  erg/s/(km/s) \\
              \texttt{L\_neg} &                                                             Luminosity of blue side &         erg/s \\
              \texttt{L\_pos} &                                                              Luminosity of red side &         erg/s \\
              \texttt{L\_tot} &                                                                    Total luminosity &         erg/s \\
      \texttt{R\_F\_cut\_neg} &       Ratio of maximum luminosity density and peak detection threshold on blue side &               \\
      \texttt{R\_F\_cut\_pos} &       Ratio of maximum luminosity density and peak detection threshold on blue side &               \\
       \texttt{R\_F\_lc\_max} &                  Ratio of luminosity density at line center and maximum peak height &               \\
      \texttt{R\_F\_pos\_neg} &                                    Ratio of luminosity density at red and blue pea. &               \\
   \texttt{R\_F\_valley\_max} &  Ratio of luminosity density in the `valley` between the peaks and the maximum peak &               \\
      \texttt{R\_L\_cut\_neg} &                           Ratio of blueward luminosity and peak detection threshold &               \\
      \texttt{R\_L\_cut\_pos} &                            Ratio of redward luminosity and peak detection threshold &               \\
      \texttt{R\_L\_pos\_neg} &                                           Ratio of redward over blueward luminosity &               \\
              \texttt{W\_std} &                                      Square-root of second moment of whole spectrum &          km/s \\
         \texttt{W\_neg\_std} &                         Blue peak width as measured by square-root of second moment &          km/s \\
         \texttt{W\_pos\_std} &                          Red peak width as measured by square-root of second moment &          km/s \\
 \texttt{neg\_peak\_fraction} &                                          Fraction of times a blue peak was detected &               \\
 \texttt{pos\_peak\_fraction} &                                           Fraction of times a red peak was detected &               \\
                \texttt{skew} &                          Pearson's moment coefficient of skewness of whole spectrum &         \\
           \texttt{skew\_neg} &                               Pearson's moment coefficient of skewness of blue side &                        \\
           \texttt{skew\_pos} &                                Pearson's moment coefficient of skewness of red side &                        \\
              \texttt{x\_max} &                      Highest peak position determined by maximum luminosity density &          km/s \\
             \texttt{x\_mean} &                                                            First moment of spectrum &          km/s \\
         \texttt{x\_neg\_max} &                 Peak position determined by maximum luminosity density on blue side &          km/s \\
        \texttt{x\_neg\_mean} &                              Peak position determined by weighted mean on blue side &          km/s \\
         \texttt{x\_pos\_max} &                  Peak position determined by maximum luminosity density on red side &          km/s \\
        \texttt{x\_pos\_mean} &                               Peak position determined by weighted mean on red side &          km/s \\
           \texttt{x\_valley} &                                              Position of `valley` between the peaks &          km/s \\
                   \texttt{z} &                                                         Systemic redshift of source &               \\
\bottomrule
\end{tabular}


